Co-design of Optimal Transmission Power and Controller for Networked Control Systems Under State-dependent Markovian Channels

This paper considers a co-design problem for industrial networked control systems to ensure both the stability and efficiency properties of such systems. The assurance of such properties is particularly challenging due to the fact that wireless communications in industrial environments are not only subject to shadow fading but also stochastically correlated with their surrounding environments. To address such challenges, this paper first introduces a novel state-dependent Markov channel (SD-MC) model that explicitly captures the state-dependent features of industrial wireless communication systems by defining the proposed model's transition probabilities as a function of both its environment's states and transmission power. Under the proposed channel model, sufficient conditions on Maximum Allowable Transmission Interval (MATI) are presented to ensure both asymptotic stability in expectation and almost sure asymptotic stability properties of a continuous nonlinear control system with state-dependent fading channels. Based on such conditions, the co-design problem is then formulated as a constrained polynomial optimization problem (CPOP), which can be efficiently solved using semidefinite programming methods for the case of a two-state state dependent Markovian channel. The solutions to such a CPOP represent optimal control and power strategies that optimize the average expected joint costs in an infinite time horizon while still respect the stability constraints. For a general SD-MC model, this paper further shows that sub-optimal solutions can be obtained from linear programming formulations of the considered CPOP. Simulation results are given to illustrate the efficacy of the proposed co-design scheme.

==> main-results-old.tex <==
\section{Main Results}
\label{sec:main-results}
This section presents the main results of this paper. Firstly, sufficient conditions on MATI are presented to ensure \emph{asymptotic stability in expectation}~(\textbf{E} in Definition \ref{def: ss})) and \emph{almost sure asymptotic stability}~(\textbf{P} in Definition \ref{def: ss})). In particular, we show that these sufficient conditions depend on the control policy used for external environment and the transmission power policy. Secondly, these sufficient conditions are used as constraints for a constrained optimization problem under which the optimal control and transmission power policies are found to minimize average costs.

The following assumptions are needed to derive the main results. 
\begin{assumption}[\cite{nesic2009explicit,carnevale2007lyapunov}]
	\label{assumption}
Consider the stochastic hybrid system in \eqref{sys:continuous} and \eqref{sys:jump}. Let $\overline{e}:=[e; \xi]$ denote an augmented vector for the error states $e$ and the size of the dynamic quantizer $\xi$. Suppose there exist a function $W : \mathbb{N}_{\geq 0} \times \mathbb{R}^{n_{e}+1} \rightarrow \mathbb{R}_{\geq 0}$ that is locally Lipschitz with respect to $\overline{e}$, a locally Lipschitz, positive definite, radially unbounded function $V: \mathbb{R}^{n_x} \rightarrow \mathbb{R}_{\geq 0}$, a continuous function $H: \mathbb{R}^{n_x} \rightarrow \mathbb{R}_{\geq 0}$, a finite set of constants $\{\lambda_{i}\}_{i=1}^{M_{R}}$, real numbers $L \geq 0, \zeta > 0$, $\underline{\alpha}_{W}, \overline{\alpha}_{W}, \underline{\alpha}_{V}, \overline{\alpha}_{V} \in \mathcal{K}_{\infty}$ and a continuous positive definition function $\varrho$ such that the followings hold:
\begin{enumerate}
	\item $\forall k \in \mathbb{N}$, $\overline{e} \in \mathbb{R}^{n_{x}+1}$ and $r_{i} \in \mathcal{R}=\{r_{1}, r_{2}, \ldots, r_{M_R}\}$
	\begin{subequations}
		\label{ineq:W}
		\begin{align}
		\underline{\alpha}_{W}(|\overline{e}|) \leq W(k, \overline{e}) &\leq \overline{\alpha}_{W}(|\overline{e}|) \\
		W(k+1, \overline{J}(k, \overline{e}, r_i)) &\leq \lambda_{i} W(k, \overline{e})
		\end{align}
	\end{subequations}
where $\overline{J}(k, \overline{e}, r_i)=[J_{e};J_{\xi}]$ with the functions $J_{e}$ and $J_{\xi}$ defined in \eqref{sys:jump}.
\item $\forall k \in \mathbb{N}, x \in \mathbb{R}^{n_x}$ and for almost all $\overline{e} \in \mathbb{R}^{n_{x}+1}$,  such that 
\begin{align}
\left\langle \frac{\partial W(k, \overline{e})}{\partial \overline{e}}, \overline{g}(x, \overline{e})  \right\rangle \leq L W(k, \overline{e})+ H(x)
\end{align}
where $\overline{g}(x, \overline{e})=[g_{e};g_{\xi}]$ with the functions $g_{e}$ and $g_{\xi}$ defined in \eqref{sys:continuous}.
	\item $\forall x \in \mathbb{R}^{n_x}$ 
	\begin{align}
	\label{ineq: alpha_V}
	\underline{\alpha}_{V}(x) \leq V(x) \leq \overline{\alpha}_{V}(x)
	\end{align}
	and $\forall k \in \mathbb{N}, \overline{e} \in \mathbb{R}^{n_{x}+1}$, and for almost all $x \in \mathbb{R}^{n_x}$
	\begin{align}
	\label{ineq:delta-V}
	\langle \nabla V(x),  \tilde{f}(x, e) \rangle \leq \varrho(|x|)-\varrho(W(k,\overline{e}))-H^{2}(x)+\zeta^{2}W^{2}(k, \overline{e})
	\end{align}
\end{enumerate}
\end{assumption}  
\begin{remark}
	
\end{remark}
\subsection{Stochastic Stability}
\label{sec:almost-sure-stability}
Under the Assumption \ref{assumption}, sufficient conditions on the MATI are presented to ensure \emph{asymptotic stability in expectation}~(Theorem \ref{thm:ase}) and \emph{almost sure asymptotic stability}~(Theorem \ref{thm:asas}) for the stochastic hybrid system defined in \eqref{sys:continuous} and \eqref{sys:jump} under the state dependent Markov channels. 
\begin{theorem}
	\label{thm:ase}
Consider the stochastic hybrid system defined in \eqref{sys:continuous} and \eqref{sys:jump}, the state-dependent Markov channel in \eqref{sys:ss-MC}, and the controlled external environment  $\mathcal{M}_{env}=\{S, S_{0}, A, Q, c\}$. Suppose Assumption \ref{assumption} holds, let $T_{MATI}$ denote the maximum allowable time interval and $\mu^{m}, \mu^{p}$ denote the stationary control and power policies respectively, the system is \emph{asymptotically stable in expectation} if 
\begin{align}
T_{MATI} \leq \begin{cases}
\frac{1}{Lr}\arctan \left(\frac{r(1-\overline{\lambda})}{2\frac{\overline{\lambda}}{1+\overline{\lambda}}(\frac{\zeta}{L}-1)+1+\overline{\lambda}} \right) \quad & \zeta > L \\
\frac{1}{L}\frac{1-\overline{\lambda}}{1+\overline{\lambda}} \quad & \zeta=L \\
\frac{1}{Lr}\arctanh \left(\frac{r(1-\overline{\lambda})}{2\frac{\overline{\lambda}}{1+\overline{\lambda}}(\frac{\zeta}{L}-1)+1+\overline{\lambda}} \right) \quad &\zeta < L
\end{cases}
\label{ineq:MATI}
\end{align}
with $r=\sqrt{\left|(\frac{\zeta}{L})^{2} -1 \right|}$ for some constant $\overline{\lambda}$ that satisfies
\begin{align}
\label{ineq:condition-lambda}
\overline{\lambda} > \sqrt{\|\diag(\lambda_{i}^{2}\mathbb{I}_{M_S})\overline{P}^{T}(\mu^{m}, \mu^{p})\|}
\end{align}
where $\overline{P}(\mu^{m}, \mu^{p})=\left[\overline{P}_{ij, mn}(\mu^{m}, \mu^{p})\right]_{1 \leq i, m \leq M_{R}, 1 \leq j, n \leq M_{S}}$ with
\begin{align*} 
&\overline{P}_{ij, mn}(\mu^{m}, \mu^{p}) \\
=&\sum_{p \in \Omega_{p}} {\rm Pr}\{\lambda_{i} \vert \lambda_{m}, s_{n}, p\}{\rm Pr}\{ p \vert \lambda_{m}, s_{n}\} \sum_{a \in A(s_n)} {\rm Pr}\{s_{j} \vert s_{n}, a\}{\rm Pr}\{a \vert s_{n}, \lambda_{m} \}.
\end{align*}
\end{theorem}
\begin{proof}
Let $\overline{x}:=[x^{T}, \overline{e}, \tau, k]^{T}$ denote an augmented state, and $F(\overline{x}):=[\tilde{f}(x, e)^{T}, \overline{g}(x, \overline{e})^{T}, 1, 0]^{T}$. Define a candidate Lyapunov function for the augmented state $\overline{x}$ as below
\begin{align}
U(\overline{x}):=V(x)+ \zeta \phi(\tau) W^{2}(k, \overline{e})
\end{align}
where the function $\phi(\tau): [0, T_{MATI}] \rightarrow \mathbb{R}$ is the solution to the following nonlinear differential equation
\begin{align}
\dot{\phi}=-2L\phi - \zeta (\phi^{2}+1), \quad \phi(0)=\overline{\lambda}^{-1}
\end{align}
Following the proof of Theorem 1 in \cite{carnevale2007lyapunov}, for all $\tau$ and $k$, we have 
\begin{align}
\langle \nabla U(\overline{x}), F(\overline{x}) \rangle \leq - \varrho(|x|) - \varrho(W(k, \overline{e})) \leq -\tilde{\varrho}(\overline{x})
\end{align}
where $\tilde{\varrho}(\overline{x})$ is a continuous and positive definition function. It then follows that there exists a class $\mathcal{KL}$ function $\beta$ such that $\forall \lambda \in \{\lambda_{i}\}_{i=1}^{M_R}$,
\begin{align}
\label{ineq:U-continuous}
U(\overline{x}(t)) \leq \beta\left(U(\overline{x}(t_{k}^{+})), t-t_{k}\right), \forall t \in [t_{k}, t_{k+1}], \forall k \in \mathbb{N}
\end{align}
Note that the randomness of the system comes from the stochastic jump equations in \eqref{sys:jump} where the sequence of the augmented state $\{\overline{e}(t_{k}^{+})\}$ is a stochastic process whose probability distribution is governed by the state-dependent Markov channel. Let $\mathbbm{1}_{A}$ denote the indicator function that takes value $1$ when sample value falls in the set $A$ and takes value $0$ otherwise. Define a set $A_{ij}:=\{\lambda_{i}, s_j\}$ with $i=1,2,\ldots, M_{R}$ and $j=1, 2, \ldots, M_{S}$ and let $U_{k+1}:=U(\overline{x}(t_{k+1}^{+}))$, then consider a vector $\overline{U}_{k+1}:=\left[\mathbb{E}[U_{k+1}\mathbbm{1}_{A_{11}}], \ldots, \mathbb{E}[U_{k+1}\mathbbm{1}_{A_{1M_{S}}}], \mathbb{E}[U_{k+1}\mathbbm{1}_{A_{21}}], \ldots, \mathbb{E}[U_{k+1}\mathbbm{1}_{A_{M_{R} M_{S}}}]\right]^{T}$ where $\forall i, j$
\begin{align}
\mathbb{E}&[U_{k+1}\mathbbm{1}_{A_{ji}}] \nonumber \\
&=\mathbb{E}[V(x(t_{k+1}^{+}))\mathbbm{1}_{A_{ij}}]+\zeta \phi(\tau^{+})\mathbb{E}[W^{2}(k+1, \overline{J}(k, \overline{e}, r))\mathbbm{1}_{A_{ij}}] \nonumber \\
&\overset{(a)}{=}V(x(t_{k+1})+\zeta \phi(0)\mathbb{E}[W^{2}(k+1, \overline{J}(k, \overline{e}, r))\mathbbm{1}_{A_{ij}}] \nonumber \\
&\overset{(b)}{\leq} V(x(t_{k+1})+\zeta \overline{\lambda}^{-1}\sum_{m=1}^{M_R}\sum_{n=1}^{M_S}\mathbb{E}[\lambda_{i}^{2} W^{2}(k, \overline{e})\mathbbm{1}_{A_{ij}}\mathbbm{1}_{A_{mn}}] \nonumber \\
&\overset{(c)}{=}V(x(t_{k+1})+\zeta \overline{\lambda}^{-1}\lambda_{i}^{2}\sum_{m=1}^{M_R}\sum_{n=1}^{M_S}{\rm Pr}\{ A_{ij} \vert A_{mn}\}\mathbb{E}[ W^{2}(k, \overline{e})\mathbbm{1}_{A_{mn}}]
\label{ineq:EU}
\end{align}
The equality $(a)$ holds due to the fact that the state $x$ is continuously evolved and is independent of the random jump caused by the Markov channel and MDP process. The inequality $(b)$ holds because of the conditions \eqref{ineq:W} in Assumption \ref{assumption}. The equality $(c)$ holds because of the \emph{state-dependent Markov channel model} defined in \eqref{sys:ss-MC} and the MDP process. Since the inequality \eqref{ineq:EU} holds for all $\lambda_{i}, s_{j}$ with $ \forall i=1,2,\ldots, M_R$, $j=1,2,\ldots, M_S$, the vector $\overline{U}_{k+1}$ satisfies 
\begin{align*}
&\overline{U}_{k+1}\leq V(x(t_{k+1}))\mathbf{e}_{M_{RS}} \\
&+ \zeta \overline{\lambda}^{-1}\underbrace{\begin{bmatrix}
\lambda_{1}^{2}\overline{P}_{11, 11} &  \lambda_{1}^{2}\overline{P}_{11, 12} & \cdots & \lambda_{1}^{2}\overline{P}_{11, M_{R} M_{S}} \\
\lambda_{1}^{2}\overline{P}_{12, 11}&  \lambda_{1}^{2}\overline{P}_{12, 12} & \cdots & \lambda_{1}^{2}\overline{P}_{11, M_{R} M_{S}} \\
\vdots & \vdots  &\vdots & \vdots \\
\lambda_{i}^{2}\overline{P}_{ij, 11}&  \lambda_{i}^{2}\overline{P}_{ij, 12} & \cdots & \lambda_{i}^{2}\overline{P}_{ij, M_{R} M_{S}} \\
\vdots & \vdots & \vdots & \vdots \\
\lambda_{M_R}^{2}\overline{P}_{M_{R}M_{S}, 11}   & \lambda_{M_R}^{2}\overline{P}_{M_{R}M_{S}, 12}  & \cdots & \lambda_{M_R}^{2}\overline{P}_{M_{R}M_{S}, M_{R}M_{S}}
\end{bmatrix}}_{\diag(\lambda_{i}^{2}\mathbb{I}_{M_S})\overline{P}^{T}(\mu^{m}, \mu^{p})} \\ 
&\times \underbrace{\begin{bmatrix}
\mathbb{E}[ W^{2}(k, \overline{e})\mathbbm{1}_{A_{11}}] \\
\mathbb{E}[ W^{2}(k, \overline{e})\mathbbm{1}_{A_{12}}] \\
\vdots \\
\mathbb{E}[ W^{2}(k, \overline{e})\mathbbm{1}_{A_{M_{R}M_{S}}}]
\end{bmatrix}}_{\overline{W^{2}}(k, \overline{e})} 
%&=V(x(t_{k+1}))\mathbf{e}_{M_R}+ \zeta \overline{\lambda}\diag(\lambda_{i}^{2})P^{T}(\mu^{m}, \mu^{p})
\end{align*} 
where $\mathbf{e}_{M_RS}:=[1, 1, \ldots, 1]^{T}$ is a column vector with $M_{RS}=M_{R}\times M_{S}$ of $1$, $\mathbb{I}_{M_{S}}$ is an identify matrix with dimension of $M_{S}$, and $\overline{P}_{ij, mn}:={\rm Pr}\{A_{ij} \vert A_{mn} \}$ with $A_{ij}=\{\lambda_{i}, s_j\}$ and $A_{mn}=\{\lambda_{m}, s_{n}\}$. The matrix $\overline{P}=[\overline{P}_{ij, mn}]$ is a transition function characterizing the transitional probabilities for the augmented states $[A_{ij}]$. Moreover, the transition matrix $\overline{P}(\mu^{m}, \mu^{p})$ is also a function of the control and transmission power policies $\mu^{m}, \mu^{p}$. Specifically, $\forall i, j, m, n$, 
\begin{align*}
&{\rm Pr}\{ \lambda_{i}, s_{j} \vert \lambda_{m}, s_{n}\} \triangleq \overline{P}_{ij, mn}(\mu^{m}, \mu^{p})\\
=&{\rm Pr}\{ \lambda_{i} \vert \lambda_{m}, s_{n}\} {\rm Pr}\{ s_{j} \vert \lambda_{m}, s_{n}\} \\
=&\sum_{p \in \Omega_{p}} {\rm Pr}\{\lambda_{i} \vert \lambda_{m}, s_{n}, p\}{\rm Pr}\{ p \vert \lambda_{m}, s_{n}\} \sum_{a \in A(s_n)} {\rm Pr}\{s_{j} \vert s_{n}, a\}{\rm Pr}\{a \vert s_{n}, \lambda_{m} \} \\
=&\sum_{p \in \Omega_{p}} P_{mi}(s_{n}, p) \mu^{p}_{p}(s_{n}, \lambda_{m}) \sum_{a \in A(s_n)} q(s_j \vert s_{n}, a) \mu^{m}_{a}(s_{n}, \lambda_{m})
\end{align*}
The first two equalities hold by applying the Bayesian law. The conditional probability ${\rm Pr}\{\lambda_{i} \vert \lambda_{m}, s_{n}, p\}$ defines the \emph{state dependent Markov channel} described in Definition \ref{def:ss-MC} and the $q(s_j \vert s_{n}, a)$ is the transition probability for the MDP process for external environments. The conditional probabilities $\mu^{m}_{a}(s_{n}, \lambda_{m}):={\rm Pr}\{a \vert s_{n}, \lambda_{m} \}$ and $\mu^{p}_{p}(s_{n}, \lambda_{m}):={\rm Pr}\{ p \vert \lambda_{m}, s_{n}\}$ are the policies for MDP process and transmission power respectively. 
 By taking the infinity norm on both sides of the above inequality, one further has
\begin{align}
&|\overline{U}_{k+1}| \nonumber \\&\overset{(d)}{\leq} V(x(t_{k+1})) +\zeta \overline{\lambda}^{-1}\|\diag(\lambda_{i}^{2}\mathbb{I}_{M_S})\overline{P}^{T}(\mu^{m}, \mu^{p})\||\overline{W^{2}}(k, \overline{e})| \nonumber \\
& \overset{(e)}{\leq} V(x(t_{k+1}))+\zeta \overline{\lambda}^{-1} \overline{\lambda}^{2}|\overline{W^{2}}(k, \overline{e})| \nonumber \\
& = V(x(t_{k+1}))+\zeta  \overline{\lambda}|\overline{W^{2}}(k, \overline{e})|\nonumber \\
& \overset{(f)}{\leq} |\overline{U}_{k}|
\label{ineq: U}
\end{align}
\end{proof}
The inequality $(d)$ holds due to the norm condition  $|y| \leq |Ax| \leq \|A\||x|$, $\forall x \in \mathbb{R}^{n}, y \in \mathbb{R}^{m}$ and $A \in \mathbb{R}^{n \times m}$. The inequality $(e)$ holds due to the condition in \eqref{ineq:condition-lambda}. The inequality $(f)$ holds by the claim that $|\overline{U}(\overline{x})|=V(x)+\zeta \phi(\tau)|\overline{W^{2}}|$. To prove the claim, note that the expectations of the positive function $U(\overline{x})$ and $W(k, \overline{e})$ are positive for all $\overline{x}, \overline{e}$. Since $\overline{U}(\overline{x})=V(x)\mathbf{e}+\zeta \phi(\tau)\overline{W^{2}}(k, \overline{e})$, one can prove the claim by noting that $|\overline{U}(\overline{x})|=|V(x)\mathbf{e}+\zeta \phi(\tau)\overline{W^{2}}(k, \overline{e})|=V(x)+\zeta \phi(\tau)|\overline{W^{2}}(k, \overline{e})|$ because $V(x), \zeta, \phi(\tau) \geq 0$ are constant with respect to the expectation operator. The condition in \eqref{ineq: U} ensures that the expected value of the Lyapunov function is non-increasing at the stochastic jump states. By the inequality \eqref{ineq:U-continuous}, we prove that the Lyapunov function $U(\overline{x})$ asymptotically decreases deterministically in-between the stochastic jumps. Thus, by combining the inequalities \eqref{ineq:U-continuous} and \eqref{ineq: U}, it is straightforward to prove that there exists a class $\mathcal{KL}$ function $\tilde{\beta}$ such that 
\begin{align}
\mathbb{E}[U(\overline{x}(t))] \leq \tilde{\beta}(U(\overline{x}(0)), t)
\end{align}
Thus, the proof is complete. 
\begin{remark}

\end{remark}
\begin{theorem}
	\label{thm:asas}
Suppose the conditions \eqref{ineq:MATI} and \eqref{ineq:condition-lambda} hold for the stochastic hybrid system in \eqref{sys:continuous} and \eqref{sys:jump}. There exist posotive constants $\underline{\alpha}_{W}, \overline{\alpha}_{W}, \underline{\alpha}_{V}, \overline{\alpha}_{V}, \varrho > 0$ such that the conditions \eqref{ineq:W}, \eqref{ineq: alpha_V} and \eqref{ineq:delta-V}  in Assumption \ref{assumption} hold with 
\begin{subequations}
	\begin{align}
		\underline{\alpha}_{W} |\overline{e}| &\leq W(k, \overline{e}) \leq \overline{\alpha}_{W} |\overline{e}| \\
			\underline{\alpha}_{V} |x|^2 &\leq V(x) \leq \overline{\alpha}_{V} |x|^2 \\
		\langle \nabla V(x),  \tilde{f}(x, e) \rangle &\leq \varrho |x|^{2}-\varrho W(k,\overline{e})-H^{2}(x)+\zeta^{2}W^{2}(k, \overline{e}). 
	\end{align}
	\label{ineq:new}
\end{subequations}
Then the stochastic hybrid system in \eqref{sys:continuous} and \eqref{sys:jump} is \emph{almost surely asymptotically stable}.
\end{theorem}

\begin{proof}
The idea of the proof is to first show that the stochastic hybrid system is \emph{exponentially stable in expectation} under the more restrictive condition in \eqref{ineq:new}. Then by the Borel-Cantelli Lemma, one can show that the \emph{exponential stability in expectation} implies the \emph{almost sure asymptotic stability} defined in \eqref{ineq:ASAS} in Definition \ref{def: ss}. To show the exponential stability in expectation, consider the Lyapunov function $U(\overline{x}):=V(x)+ \zeta \phi(\tau) W^{2}(k, \overline{e})$ and the following inequality holds for each transmission time interval, i.e., $\forall \tau \in [0, T_{MATI}]$, 
\begin{align*}
\langle \nabla U(\overline{x}), F(\overline{x}) \rangle &\leq - \varrho |x|^{2} - \varrho W(k, \overline{e}) 
\leq - \varrho |x|^{2} - \varrho \overline{\alpha}_{W} |\overline{e}|^2 \\
& \leq -(\varrho+\varrho \overline{\alpha}_{W})*(|x|^{2}+|\overline{e}|^2) = -\tilde{\varrho} |\overline{x}|^{2}
\end{align*}
with $\tilde{\varrho}=\varrho+\varrho \overline{\alpha}_{W}$. By the conditions in \eqref{ineq:new}, it is straightforward to show that the $\underline{\alpha}_{U} |\overline{x}|^{2} \leq U(\overline{x}) \leq \overline{\alpha}_{U} |\overline{x}|^{2}$ with the positive constants $\underline{\alpha}_{U}=\underline{\alpha}_{V}+\zeta \overline{\lambda}	\underline{\alpha}_{W}$ and $ \overline{\alpha}_{U}=\overline{\alpha}_{V}+\zeta \overline{\lambda}^{-1} \overline{\alpha}_{W}$ where $\overline{\lambda}$ is defined in \eqref{ineq:condition-lambda}. Then, one can show that $U(\overline{x}(t, k)) \leq \exp\left(-\frac{\tilde{\varrho} }{\overline{\alpha}_{U}}(t-t_k)\right) U(\overline{x}(t_k, k)), \forall k \in \mathbb{N}, t-t_k \in [0, T_{MATI}]$. Moreover, Theorem \ref{thm:ase} shows that $\mathbb{E}[U(\overline{x}(t, k+1))] \leq \mathbb{E}[U(\overline{x}(t, k))], \forall k \in \mathbb{N}$ if the condition in \eqref{ineq:condition-lambda} holds. By combining the dynamics of both the continuous and discrete flows of the stochastic hybrid system proved above, one can show that $\mathbb{E}[U(\overline{x}(t, k))] \leq \exp\left(-\frac{\tilde{\varrho} }{\overline{\alpha}_{U}} t \right) U(\overline{x}(0, 0))$ which implies that $\mathbb{E}[|\overline{x}(t, k)|^{2}] \leq \exp\left(-\frac{\tilde{\varrho} }{\overline{\alpha}_{U}} t \right) \frac{\overline{\alpha}_{U}}{\underline{\alpha}_{U}} |\overline{x}(0,0)|^{2}$. Following the proof of Theorem 9 in \cite{hu2019co}, one can show that the \emph{exponential stability in expectation} implies the \emph{almost sure asymptotic stability} by using the Borel-Cantelli Lemma. Please refer to \cite{hu2019co, hu2019optimal} for the details of the proof. 
%one needs to show that the following conditions hold for some positive constants $\underline{\alpha}_{U}, \overline{\alpha}_{U}, \delta_{U} > 0$
%\begin{subequations}
%	\begin{align}
%	\underline{\alpha}_{U} |\overline{x}_{c}|^{2} \leq U(\overline{x}) &\leq \overline{\alpha}_{U} |\overline{x}_{c}|^{2} \\
%    \langle \nabla V(\overline{x}),  F(\overline{x}) \rangle &\leq -\delta_{U} |\overline{x}_{c}|^{2},  \forall \tau \in [0, T_{MATI}] \label{ineq:U-c}\\
%    \mathbb{E}\left[U(F(\overline{x})) \vert U(\overline{x})\right] &\leq U(\overline{x}), \forall k \in \mathbb{N} \label{ineq:U-d}
%	\end{align}
%	\label{ineq:U}
%\end{subequations}
%The inequality \eqref{ineq:U-c} is related to the exponentially decreasing condition of the continuous dynamics of the stochastic hybrid system. The supermartingale condition \eqref{ineq:U-d} implies that the conditional expectation of the Lyapunov function $U$ is not increasing at the jumps of the hybrid system.  Since $U(\overline{x}):=V(x)+ \zeta \phi(\tau) W^{2}(k, \overline{e})$, one has 

\end{proof}
\begin{remark}
\end{remark}
\subsection{Optimal Co-design of Control and Power Policies: A Constrained Optimization Problem}
\label{sec:noncooperative-game}
This section formulates the optimal co-design problem of control and power policies as a constrained optimization where the stability condition in \eqref{ineq:condition-lambda} serves as the constraint. As shown in Problem \ref{problem-efficiency}, optimal stationary control and power policies are seek to minimize a joint average cost under the stability condition. The following theorem shows that the co-design problem proposed in Problem \ref{problem-efficiency} can be reformulated as a quadratically constrained quadratic program. In particular, the stability conditions given in \eqref{ineq:condition-lambda} can be written as quadratic constraints. 
\begin{theorem}
	\label{thm:qcqp}
Let $\mu^{p^{*}}$ and $\mu^{m^{*}}$ denote the optimal stationary control and power policies for the co-design problem formulated in \ref{ineq:ASAS}, the optimal control and power policies can be equivalently obtained by solving the following quadratic program. 
	\begin{subequations}
\label{opt: qcqp}
\begin{alignat}{5}
&\!\min_{X(s, a, r, p)} & & \sum_{s \in S, p \in \Omega_{p}, r \in \mathcal{R}, a \in A}\left(c_{M}(s, a)+ \eta c_{P}(p, r) \right)X(s, a, r, p) \label{opt: obj}\\
& \text{s.t.}
& & \sum_{a \in A(s)} X(s, a)-\sum_{\substack{a \in A(s) \\ s' \in S}}q(s \vert s', a)X(s', a), \forall s \in S \label{opt: mdp1} \\
& &  &\sum_{\substack{ s\in S \\ p \in \Omega_{p}}} X(s, r, p)-\sum_{\substack{p \in \Omega_{p} \\ s \in S \\ r' \in \mathcal{R}}} {\rm Pr}\{ r \vert r', s, p \}X(r', s, p), \forall r \in \mathcal{R} \label{opt: mdp2} \\
& & &\sum_{s \in S, p \in \Omega_{p}, a \in A(s), r \in \mathcal{R}}X(s, a, r, p)=1 \label{opt: occupation} \\
& & &\sum_{m=1}^{M_{R}}\sum_{n=1}^{M_{s}} \frac{\sum_{p \in \Omega_{p}}P_{mi}(s_{n}, p)X(s_{n}, r_{m}, p)}{X^{2}(s_{n}, r_{m})} \nonumber \\
& & & \times \sum_{a \in A(s_{n})}Q_{nj}(a)X(s_{n}, r_{m}, a)< \theta_{i}^{2}, \forall i=1,2,\ldots, M_{R} \label{opt: stability}
\end{alignat}
\end{subequations}
where $\theta_{i}=\overline{\lambda}/\lambda_{i}$ and $Q_{nj}(a)=q(s_{j}| s_{n}, a)$ that is a transition probability defined in the MDP system. The optimal policies $\mu^{p^{*}}$ and $\mu^{m^{*}}$ can then be represented as below
\begin{align}
\mu^{p^{*}}_{p}(r, s)={\rm Pr}\{p \vert r, s\}=\frac{\sum_{a \in A(s)}X^{*}(s, r, a, p)}{\sum_{a \in A(s), p \in \Omega_{p}}X^{*}(s, r, a, p)} \\
\mu^{m^{*}}_{a}(r, s)={\rm Pr}\{a \vert r, s\}=\frac{\sum_{p \in \Omega_{p}}X^{*}(s, r, a, p)}{\sum_{a \in A(s), p \in \Omega_{p}}X^{*}(s, r, a, p)}
\end{align}
where $\{ X^{*}(s, r, a, p)\}_{s \in S, r \in \mathcal{R}, a \in A(s), p \in \Omega_{p}}$ are the solutions to the quadratic program.  
\end{theorem}
\begin{proof}
Please refer to the Appendix \ref{appendix} for the proof. 
\end{proof}
\begin{remark}
	
\end{remark}


==> problem-formulation-revised.tex <==
\section{System Description}
\label{sec:problem-formulation}
This paper considers a nonlinear physical system controlled over a state-dependent Markov channel. As depicted in Fig. \ref{fig: sys}, the system framework consists of a \emph{nonlinear plant}, a \emph{state-dependent Markov channel}, a \emph{remote controller} and the \emph{external environment} that is modeled by a Markov Decision process. Each part of the system will be detailed in the following sections. 
\begin{figure}[!t]
	\centerline{\includegraphics[width=\columnwidth]{fig/system}}
	\caption{Nonlinear Networked Control System with State-dependent Markov Channels}
	\label{fig: sys}
\end{figure}

\subsection{System Model}

The dynamics of the nonlinear plant are modeled by the following ODE
\begin{align}
\label{sys:nonlinear}
\dot{x}=f(x, u)
\end{align}
where $x \in \mathbb{R}^{n_{x}}$ is a vector representing the states of the nonlinear plant, $u \in \mathbb{R}^{n_u}$ is the control input. The function $f: \mathbb{R}^{n_{x}} \times \mathbb{R}^{n_u}  \rightarrow \mathbb{R}^{n_{x}}$ is the vector field of the nonlinear system. The state information $x$ is used by a controller to generate control action $u$ that is applied to the plant. In this paper, we assume that the state information $x$ can be accessed by the controller through a \emph{state-dependent} wireless communication channel.  

The state information $x$ is not perfectly known to the controller due to the presence of the wireless communication channel. This paper considers both the sampling and quantization effects on the state information $x$.  Specifically, let $\{t_{k}\}_{k=0}^{\infty}$ denote a sequence of sampling time instants with $t_{k} < t_{k+1}$, then the state at a time instant $t_k$ can be represented by $x_{k}:=x(t_{k})$. The sampled state $x(t_k)$ is then encoded by one of a finite number of symbols, and transmitted through the communication channel. The finite number of symbols are constructed by a dynamic quantization scheme discussed in the following subsection. 
\subsection{Dynamic Quantized Control System}
Similar to the framework in \cite{nesic2009unified}, the dynamic quantization scheme considered in this paper is a function that maps the sampled state $x \in \mathbb{R}^{n_x}$ into the index of a finite number of symbols. Specifically, let $R \in \mathbb{N}$ denote the number of bits used to construct the symbol, and the sequence of the symbols can then labeled as $\mathcal{S}=\{1, 2, \ldots, 2^{R}\}$ with a total number of $2^{R}$. The way of using the symbol to encode the state information $x(t_k)$ is by constructing a dynamic quantizer that is able to track the evolution of the $x(t_k)$ at each transmission instant. The quantizer is defined as a tuple $\mathcal{Q}=(\mathcal{S}, q(\cdot), \xi)$ where $q(\cdot):\mathbb{R}^{n_x} \rightarrow \mathcal{S}$ is a quantization function that maps the system state into the symbol and $\xi \in \mathbb{R}_{\geq 0}$ is an anxiliary variable defining the size of the quantization regions. One typical method to implement the quantizer $\mathcal{Q}$ is the construction of a hybercubic box that is evolved dynamically to contain and track the state $x$. To demonstrate the mechanism of such box-based dynamic quantizer, suppose a hypercubic box is constructed at time instant $t_k$ with $\hat{x}(t_k)$ denoted as the center of the box and $2\xi(t_k)$ as its size. Then, the box is divided equally into $2^{R}$ smaller sub-boxes with each sub-box labeled as one of the symbols $\mathcal{S}$. Among all the symbols, let $q(x) \in \mathcal{S}$ denote the symbol (sub-box) that contains the state information $x$. The center of that sub-box, $\hat{x}(t_k^{+})$, is then used as an updated estimate of the state information $x$ at time instant $t_k$. The hyper-cubic box is then updated with a new center $\hat{x}(t_{k}^{+})$ and a new size $\xi(t_{k}^{+})=\xi(t_{k})/2^{R}$. The symbol representing this updated hyber-cubic is transmitted through the wireless communication channel. The following equations are used to characterize the dynamics of the dynamic quantizer 
\begin{subequations}
	\label{sys:quantizer}
\begin{align}
\hat{x}(t_{k}^{+})&=h(k, q(x(t_k)), \hat{x}(t_k), \xi(t_k), R_k) \\
\xi(t_{k}^{+})&=\frac{\xi(t_{k})}{2^{R_k}}
\end{align}
\end{subequations}
where $R_{k}$ is the number of bits available at time instant $t_k$, and can be changed at different time instants. In the following subsection, this paper will introduce a \emph{state-dependent Markov Channel Model} that characterizes both the time varying nature and the \emph{state-dependent} feature of the data rate $R_k$ in complex industrial environments.  As discussed in prior work \cite{nesic2009unified,liberzon2005stabilization}, within each time interval $[t_k, t_{k+1}), \forall k \in \mathbb{Z}_{\geq 0}$, the size of the hyper-cubic box needs to be propagated to ensure that the constructed box captures the actual state $x$. To be specific, we define the following differential equation to characterize the evolution of the size over time 
\begin{align}
\dot{\xi}(t)=g_{\xi}(\xi), \forall t \in  [t_k, t_{k+1})
\label{eq:box-size}
\end{align}

Under the dynamic quantizer $\mathcal{Q}$, this paper considers a model-based remote controller that maintains a "copy" of the plant dynamics in \eqref{sys:nonlinear} defined as below,
\begin{align}
\label{sys:controller}
\dot{\hat{x}}&=f(\hat{x}, u), \nonumber \\
u&=\kappa(\hat{x}),  \forall t \in [t_k, t_{k+1}) 
\end{align}
with the initial state $\hat{x}(t_{k})=\hat{x}(t_{k}^{+})$ over the time interval $[t_k, t_{k+1})$. The control function $\kappa(\cdot):\mathbb{R}^{n_x} \rightarrow \mathbb{R}^{n_u}$ is a "nominal" controller that is selected to stabilize the dynamic system in \eqref{sys:controller} without considering the effect of the network. 

With the definitions of system dynamics in \eqref{sys:nonlinear}, dynamic quantizer in \eqref{sys:quantizer} and \eqref{eq:box-size}, and remote controller in \eqref{sys:controller}, the closed loop system can be characterized as a stochastic hybrid system defined as below,
\begin{subequations}
	\label{sys:continuous}
	\begin{align}
	\dot{x}&=\tilde{f}(x, e) \\
	\dot{e}&=g_{e}(x, e) \\
	\dot{\xi}&=g_{\xi}(\xi), \forall t \in (t_k, t_{k+1}) 
	\end{align}
\end{subequations}
and 
\begin{subequations}
	\label{sys:jump}
	\begin{align}
	e(t_{k}^{+})&=J_{e}(k, x(t_k), e(t_k), \xi(t_k), R_k) \\
	\xi(t_{k}^{+})&=J_{\xi}(\xi(t_k), R_k), \forall k \in \mathbb{Z}_{\geq 0}
	\end{align}
\end{subequations}
where $e:=x-\hat{x}$ is the estimation error and $\tilde{f}(x, e)=f(x, \kappa(x-e))$, $g_{e}(x, e)=f(x, \kappa(x-e))-f(x-e, \kappa(x-e))$, $J_{e}(k, x(t_k), e(t_k), \xi(t_k), R_k)=x(t_k)-h(k, q(x(t_k)), x(t_k)-e(t_k), \xi(t_k), R_k)$ and $J_{\xi}=\xi(t_k)2^{-R_k}$. The equations \eqref{sys:continuous} above characterize the continuous dynamics of the closed loop system while the equations \eqref{sys:jump} describe the stochastic jump behavior of the system whose dynamics are governed by the time varying data rate $R_k$. This paper models the fading channels as a \emph{state-dependent Markov chain} that is described in the following section.

%\subsection{Controlled External Environment: A MDP Framework}

\subsection{State-dependent Markov Channel Model} 
This paper explicitly considers impact of the external environment on the wireless communication channels. To be specific, the channel conditions~(reflected by the time varying data rate $R_k$ in this paper) are changed as a function of the environment states, which can be modeled as a Markov Decision Process. The MDP framework is used to model the scenarios when the external environments can be controlled to some extent by selecting different actions. One typical example is the warehouse application where the movement of large size vehicles, such as forklifts, blocks the transmission signals of the senor networks co-existed and shared in the same space. This phenomenon is well known as shadow fading effects that exist in many industrial wireless communication networks. The big difference between the work proposed in this paper and prior literature lies in the fact that the external environments considered in this paper can be controlled while the other existing work often treats external environments as noises or disturbance that cannot be controlled. This difference leads to a novel constrained non-cooperative game framework proposed in the next section to address both the stability and efficiency issues in industrial networked systems. The controlled external environment is a MDP with $\mathcal{M}_{env}=\{S, s_{0}, A, Q\}$ where $S=\{s_{i}\}_{i=1}^{M_s}$ is a finite set of environment states, $s_0$ is an initial state, $A=\{a_{i}\}_{i=1}^{M_a}$ is a finite set of actions, and $Q=\{q(s|s', a)\}_{s, s' \in S, a \in A}$ is a transition matrix.

%\begin{example}[Forklift and Senor Networks]
%\label{example-state-dependent}
%\end{example}

Let the sequence $\mathcal{I}=\{t_{k}\}_{k=0}^{\infty}$ denote the transmission time instants, the data rates $\{R_{k}\}_{k=0}^{\infty}$ over these transmission time instants form a random process that characterizes the stochastic variations on the channel conditions. At each time instant $t_k$, we assume that the communication system can select different transmission power levels to send the data through the wireless communication channels. The transmission power can be selected from a pre-defined group of power levels. Let $\Omega_{p}=\{1, 2, \ldots, M_p \}$ denote a finite set of $M_p$ transmission power levels with $i \in \Omega_{p}$ representing the power level $i$. We assume that the strength of the transmission power is increased with a higher power level selected. Let $p_{k}:=p(t_{k}) \in \Omega_{p}$ denote the power level selected at time instant $t_k$. Then, with the controlled external environment MDP this paper considers a \emph{state-dependent Markov Channel} defined as below
\begin{definition}
	\label{def:ss-MC}
Given a power set $\Omega_{p}$, a dynamical environment modeled by a MDP $\mathcal{M}_{env}$ and a finite set of data rates $\mathcal{R}=\{r_{1}, r_{2}, \ldots , r_{M_{R}}\}$ where the data rates are arranged in an ascending fashion, i.e., $r_{i} < r_{j}, \forall i < j$, a wireless communication channel is a \emph{state-dependent Markov Channel} if $\forall s \in S, p\in \Omega_{p}$ and $\forall r_{i}, r_{j} \in \mathcal{R}$
\begin{align}
\label{sys:ss-MC}
\mathbb{P}\{R_{k+1}=r_i | R_{k}=r_{j}, s_{k}=s, p_{k}=p\}=P_{ij}(s, p)
\end{align}
where $P_{ij}(s, p)$ is a transition probability from data rate $r_{j}$ to $r_{i}$ given the transmission power $p$ and environment state $s$. 
\end{definition} 
The \emph{state-dependent Markov channel} model in \eqref{sys:ss-MC} can be viewed as a generalization of traditional Markov channel that ignores the impact of environment state and transmission power \cite{minero2012stabilization,zhang1999finite}. The Example \ref{example-ss-MC} shows how the \emph{state-dependent Markov channel model} proposed in \eqref{sys:ss-MC} can be derived from classic estimation methods in \cite{zhang1999finite,goldsmith1997variable} that generates the conventional Markov channel model. From technical standpoint, the following example demonstrates the generality of the state-dependent Markov channel model proposed in this paper. 
\begin{example}
	\label{example-ss-MC}
The characterization of \emph{state-dependent Markov channel model} in \eqref{sys:ss-MC} is an abstraction of temporal channel state variations under different transmission power and external environments. The received SNR is a function of the transmission power and environment states. To explicitly show the impact of such state-dependent features on the received SNR, suppose the (small scale)~channel gain follows a Raleigh distribution with $Rayleigh(1)$\footnote{The example selects unit parameter $Rayleigh(1)$ for the sake of notation simplicity and the channel model proposed in \eqref{sys:ss-MC} can be applied to other parameters and distributions.} and let $\varphi: S \rightarrow [0, 1]$ denote a function that characterizes the impact of different environment states $s \in S$ on the shadow fading effect, the received instantaneous SNR $\gamma$ under the transmission power $p \in \Omega_{p}$ and the environment state $s \in S$ is a random variable that follows an exponential distribution with probability density function 
\begin{align}
f_{d}(\gamma)=\frac{1}{\overline{\gamma}}\exp\left(-\frac{\gamma}{\overline{\gamma}}\right), \gamma \geq 0.
\end{align}
where $\overline{\gamma}=\frac{p\varphi(s)}{N_{0}B}$ is the average SNR with $N_0$ and $B$ representing the noise density and the received signal bandwidth respectively. The states of $M_{R}$ data rates in the Markov channel are obtained by partitioning the received SNR into $M_{R}$ disjoint intervals $\cup_{i=1}^{M_{R}} [\Gamma_i, \Gamma_{i+1})$ with $\Gamma_{i}$ and $\Gamma_{i+1}$ representing the low and high thresholds, respectively for the interval $i$. For each interval, there is one selected data rate $r \in \mathcal{R}$ to ensure sufficiently small bit error rate \cite{zhang1999finite}. Thus, we say that the data rate is $r_i$ if the received SNR values are located in the corresponding interval. Based on the results in \cite{zhang1999finite}, the transition probability can be approximated as 
\begin{align}
\label{exp-tp}
P_{i, i+1}=\frac{N_{i+1}T_p}{\pi_{i}}, P_{i,i-1}=\frac{N_{i}T_p}{\pi_{i}}, P_{ii}=1-P_{i, i+1}-P_{i,i-1}.
\end{align}
where\footnote{The parameter $f_{D}$ is the maximum Doppler frequency and $T_p$ is the one packet time period.} $N_{i}=\sqrt{\frac{2\pi \Gamma_{i}}{\overline{\gamma}}}f_{D}\exp\left(-\frac{\Gamma_{i}}{\overline{\gamma}} \right)$ and $\pi_{i}={\rm Pr}\{\Gamma_{i} \leq \gamma \leq \Gamma_{i+1}\}=\exp\left(-\frac{\Gamma_i}{\overline{\gamma}}\right)-\exp\left(-\frac{\Gamma_{i+1}}{\overline{\gamma}}\right)$. Since $\overline{\gamma}=\frac{p\varphi(s)}{N_{0}B}$, the transition probabilities defined in \eqref{exp-tp} change as a function of the transmission power $p$ and environment states $s$. 
\end{example}

As shown in \eqref{sys:ss-MC}, the \emph{state-dependent} Markov channel can be somewhat manipulated by selecting transmission power and controlling environment to appropriate states. Such \emph{state-dependency} feature captures the fundamental correlations among different systems in industrial environments, which has been studied and verified in many experimental results, such as \cite{agrawal2014long,kashiwagi2010time}. However, few work has explored such unique feature to ensure system stability and efficiency. One of the main contributions of this paper is to develop a constrained non-cooperative game framework under which the system stability and efficiency can be guaranteed in the presence of \emph{state-dependent Markov channels}.
\section{Problem Formulation}
Given the closed-loop networked control system represented by \eqref{sys:continuous}, \eqref{sys:jump} and \eqref{sys:ss-MC}, one of the problem of interest is to ensure that the system is stochastically stable. The notions of \emph{stochastic stability} is formally defined in Definition \ref{def: ss}.
\begin{definition}[Stochastic Stability \cite{khasminskii2011stochastic}]
\label{def: ss}
the closed-loop networked control system represented by \eqref{sys:continuous} and \eqref{sys:jump} under the \emph{state-dependent Markov channel} modeled by \eqref{sys:ss-MC},
	\begin{itemize}
	\item[\textbf{E}] The system is said to be \emph{asymptotically stable in expectation} (ASE) if there exist a class $\mathcal{KL}$ function $\beta(\cdot, \cdot)$ and a bounded set $\Omega_{r}=\{ x \in \mathbb{R}^{n} : |x| <  r \}$ such that for all $x_{0} \in \Omega_{r}$:
	\begin{align}
	\label{ineq:ASE}
	\mathbb{E}(|x(t)|) \leq \beta(|x_0|, t-t_0),   \quad \forall t \in \mathbb{R}_{\geq 0}
	\end{align}
	and that $\lim_{t \rightarrow \infty}\mathbb{E}(|x(t)|)=0$.
	\item[\textbf{P}] The system is said to be \emph{almost surely asymptotically stable} (ASAS) if $\forall \epsilon, t' > 0$, such that:
	\begin{align}
	\label{ineq:ASAS}
	\mathbb{P}\{\lim_{t' \rightarrow \infty}\sup_{t \geq t'}|x(t)| \geq \epsilon \} = 0
	\end{align}
\end{itemize}
\end{definition}
\begin{remark}
The ASAS is a stronger stability notion than the ASE in the sense that the former implies the latter while the ASE normally does not lead to the ASAS. As a matter of fact, one can prove that the system is ASAS if it is \emph{exponentially stable in expectation} where there exists an exponential function $\beta(|x_0|, t-t_0):=c_{1}\exp\big(-c_{2}(t-t_{0})\big)|x_0|$ with $c_{i} > 0, \forall i=1, 2$ such that the inequality \eqref{ineq:ASE} holds \cite{hu2019co, hu2019optimal}. 
\end{remark}
\begin{problem}[Stability Problem]
	\label{problem-stability}
	The first problem of this paper is to find the Maximum Allowable Transmission Time Interval~(MATI) under which the networked control system with \emph{state-dependent Markov channels} satisfies the notions of stochastic stability defined in Definition \ref{def: ss}.
\end{problem}
\begin{problem}[Efficiency Problem]
	\label{problem-efficiency}
Let $\mu_{m}$ and $\mu_{p}$ denote the control policy and transmission power policy respectively, and for a given joint cost function $\{c(s, p, r)\}_{s \in S, p \in \Omega_{p}, r \in \mathcal{R}}$ the second problem is to find an optimal policy $\mu^{\star}:=(\mu^{\star}_{m}, \mu^{\star}_{p})$ such that the following average expected costs are minimized under the stability conditions from Problem \ref{problem-stability},
	\begin{equation}
	\label{opt: game-1}
	\begin{aligned}
	& \underset{\mu_{m}, \mu_{p}}{\text{min}}
	& & J(\{s_{0}, R_{0}\}, \mu_{m}, \mu_{p})=\lim_{T \rightarrow \infty}\frac{1}{T} \mathbb{E}_{s_{0}, R_{0}}^{\mu_{m}, \mu_{p}} \sum_{i=0}^{T} c(s_{k}, p_{k}, R_{k})\\
	& \text{s.t.}
	& & \text{Stability conditions ensuring } \eqref{ineq:ASE} \text{ or } \eqref{ineq:ASAS}
	\end{aligned}
	\end{equation}
	where $s_{0}$ and $R_{0}$ are initial states for the MDP system and Markov channel respectively. 
\end{problem}

This paper first derives sufficient conditions on MATI to ensure stochastic stability notions defined in Definition \ref{def: ss}. These stability conditions serve as constraints in the optimization problem formulated in \eqref{opt: game-1}.
